Leveraging SE(3) Equivariance for Self-Supervised Category-Level Object Pose Estimation

Category-level object pose estimation aims to find 6D object poses of previously unseen object instances from known categories without access to object CAD models. To reduce the huge amount of pose annotations needed for category-level learning, we propose for the first time a self-supervised learning framework to estimate category-level 6D object pose from single 3D point clouds.During training, our method assumes no ground-truth pose annotations, no CAD models, and no multi-view supervision. The key to our method is to disentangle shape and pose through an invariant shape reconstruction module and an equivariant pose estimation module, empowered by SE(3) equivariant point cloud networks.The invariant shape reconstruction module learns to perform aligned reconstructions, yielding a category-level reference frame without using any annotations. In addition, the equivariant pose estimation module achieves category-level pose estimation accuracy that is comparable to some fully supervised methods. Extensive experiments demonstrate the effectiveness of our approach on both complete and partial depth point clouds from the ModelNet40 benchmark, and on real depth point clouds from the NOCS-REAL 275 dataset. The project page with code and visualizations can be found at: https://dragonlong.github.io/equi-pose.

==> table/04_nocs_real.tex <==
\begin{table*}[t]
\caption{
%
\textbf{6D pose evaluation on NOCS-REAL 275 dataset.} Here we show translation error is in m and we keep the other two metrics the same to Table 2.
% We also show the unidirectional chamfer L1 loss for the matchness of generated canonical shape. 
%
}
\label{tab:nocs}
\centering
\resizebox{1\linewidth}{!} 
{
\begin{tabular}{c cccccc}
%
\toprule
%
$R_{err}$ $\downarrow$ / $T_{err}$ $\downarrow$ / Acc. $\uparrow$ & Camera & Laptop & Mug & Bottle  & Bowl & Can \\
%
\midrule
1) &
39.49 / \textbf{0.05} / 0.06 &
\textbf{4.06} / 0.03/ 0.55 &
\textbf{4.75} / 0.04 / \textbf{0.53} &
3.01 / \textbf{0.03} / 0.78 &
\textbf{3.45}/ \textbf{0.04} / \textbf{0.73} &
2.41/ \textbf{0.04} / 0.86 &
\\

2) & 
\textbf{15.26} / 0.08 / \textbf{0.07} &
8.10 / \textbf{0.02} / 0.39&
5.03 / \textbf{0.03} / 0.49&
\textbf{2.60} / 0.07 / \textbf{0.86} &
5.14 / 0.04 / 0.48 &
2.52 /0.13 / \textbf{0.87} &
 
\\
3) & 
167.75 / 0.06 / 0.0 &
13.64 / 0.06 / 0.01 & 
126.62 / 0.22 / 0.0 & 
4.53/0.05/0.57 &
7.52 / 0.04 / 0.22 & 
3.88 / 0.13 / 0.68 & 

\\
4) & 


79.18/0.07/0.00 &
5.32/0.02/48.38 &

134.29/0.12/0.04 &
3.51/0.05/0.72 &
5.94/0.08/0.38 &
2.68/0.16/0.87 &

\\
5) & 
115.75 / 0.11 / 0 &
22.13 / 0.12 / \textbf{0.72} & 
127.31 / 0.07 / 0.35 &
22.13 / 0.12 / 0.72 & 
9.93 / 0.06 / 0.20 & 
\textbf{2.27} / 0.08 / 0.89 & 
\bottomrule
%
\end{tabular}
}
\vspace{-5mm}
\end{table*}

==> tex/05_ablations.tex <==




==> tex/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{supplementary material}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{in the section of conclusion.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{supplementary material}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{supplementary material}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
